3D-FFS: Faster 3D object detection with Focused Frustum Search in sensor fusion based networks

In this work we propose 3D-FFS, a novel approach to make sensor fusion based 3D object detection networks significantly faster using a class of computationally inexpensive heuristics. Existing sensor fusion based networks generate 3D region proposals by leveraging inferences from 2D object detectors. However, as images have no depth information, these networks rely on extracting semantic features of points from the entire scene to locate the object. By leveraging aggregated intrinsic properties (e.g. point density) of point cloud data, 3D-FFS can substantially constrain the 3D search space and thereby significantly reduce training time, inference time and memory consumption without sacrificing accuracy. To demonstrate the efficacy of 3D-FFS, we have integrated it with Frustum ConvNet (F-ConvNet), a prominent sensor fusion based 3D object detection model. We assess the performance of 3D-FFS on the KITTI dataset. Compared to F-ConvNet, we achieve improvements in training and inference times by up to 62.80% and 58.96%, respectively, while reducing the memory usage by up to 58.53%. Additionally, we achieve 0.36%, 0.59% and 2.19% improvements in accuracy for the Car, Pedestrian and Cyclist classes, respectively. 3D-FFS shows a lot of promise in domains with limited computing power, such as autonomous vehicles, drones and robotics where LiDAR-Camera based sensor fusion perception systems are widely used.

==> textdump.tex <==
% --------------- ABSTRACT STUFF -------------------- 

%  In this work we propose a novel heuristic for optimizing the search space for sensor fusion based advanced 3D object detection models. Existing sensor fusion models generate 3D region proposals by leveraging inferences from 2D object detectors. However, as images have no depth information, existing fusion based models rely on extracting features from the entirety of the mapped 3D space to detect objects. By leveraging intrinsic properties of the 3D point cloud data, we approximate the depths of the objects of interest in a scene and thereby substantially narrow down the 3D search space. Our heuristic is lightweight and can be incorporated across a wide range of sensor fusion based 3D detection models. To demonstrate its efficacy, we have integrated it with Frustum Convnet (F-ConvNet), a state of the art 3D object detection model. We have achieved x\% accuracy on the KITTI Validation set (B class), which is y\% better than the original F-ConvNet model. Moreover, our proposed approach improves the inference and training times of F-ConvNet by z\% and a\%, respectively.   


% Only 3D or just 2D is not ideal for object detection in all use cases and as a result 2D-3D sensor fusion has become increasing popular. The main advantage of 2D detectors are that they are reliable and highly accurate. However, when we convert the domain from 2D to 3D we are essentially increasing the dimensionality or DOF by 1, meaning each pixel can correspond to any arbitrary depth. Most of the existing industry is already equipped with camera, but that object detection cannot easily infer depth of any object. To better acquire this information LIDAR is increasingly being used. Although we can easily project 3D points into 2D image (reducing dimension), the reverse process is non trivial (going to a higher dimension). In order to locate the right solution (find the depth), existing solutions use some kind of grid search. As many of the applications using 3D sensors (ADAS, AV etc) are also equipped with camera, it is cheaper/convenient to levarage 2D detectors to classify objects. However we still need 3D for precise object detection. This is why sensor fusion is getting increasingly popular in industry and academia. 

% Our setup is compatbile with existing capabiltiies/infrastrcuture in the AV/Autonomous robotics industry and we are simply levaraging some of these capabiltiies to improve runtime/performance/capacity etc. 

% Tracking the object in the 3D scene is inefficient, for which we use a LIDAR or Point Cloud sensor. In sensor fusion approaches, we try to detect an object in 2D and try to precisely localize it in 3D. We want to improve the performance of such systems and remove the search bottleneck...The methodology we are using is a heuristic which uses intrinsic properties of the 3D point cloud instead of per point basis semantic information. As a result our process is faster/more efficient blah blah. If we have a 2D-3D setup (described in depth later) we can harness/leverage the learning/information from 2D detector to locate  the object in 3D and reduce the amount of computation/search we need to by using the intrinsic properties of 3D data...

% Simpler/Intrinsic properties such as point density can be used as a indicator to identify the region of interest and narrow down our search space. We experimented with multiple properties and heuristics in order to perform this search space reduction. One of the promising heuristics we explore uses point cloud density at various regions to generate a depth estimation inside the 3D Frustum in order to reduce search space. These heuristics are computationally cheaper and simpler and can be run without GPU/High performance machines etc. Mention the heuristics you explored. 

% As a motivating example we use a state of the art 3D detection model called F-ConvNet and integrate our heuristic search approach in this architecture. and describe your experimental results without impacting the accuracy etc. 

% clarify that our contribution is we are using some heuristics to reduce the search space that is easy/fast/does not need semantic information. 






% 3D object detection has gained increasing attention from the scientific community due to its wide-ranging applications in various domains such as autonomous driving vehicles and robotics. In this study, we present a high-performance meta-method to facilitate 3D object detection using 2D images and 3D point clouds. %Due to the inability of conventional cameras in 3D scene perception, 3D sensors such as LiDAR sensors are attracting considerable interest from both industry and academia. 
% Typically, object region proposals in 2D are used to generate frustums in the 3D point cloud which are subsequently processed further using 3D deep learning networks. Considering the entire depth of a frustum as the 3D search space is computationally challenging and have downstream impact on 3D object detection. Different regions in a particular frustum may result in differential and perhaps in some cases less desirable outcomes both in terms of accuracy and running time. Thus, fundamental to the success of this approach is to efficiently localize objects in point clouds of region proposals. Therefore, the application of frustum-based approaches to real-time object detection is riddled with their computational challenges in searching through the entire depth of the frustum. In this study, we have proposed a method to use heuristics to bound/identy the region of interest inside a frustum to effectively capture a \textit{region-of-interest} and thereby substantially pruning the 3D search space.
% This simple yet effective heuristic leverages the RGB and 3D point cloud information to generate depth estimation for the objects of interest in different frustums. Based on these center estimates of the objects of interest, we bound the near and far planes of the frustums to a constrained region-of-interest. We have demonstrated the efficacy of our proposed approach by integrating this to the Frustrum ConvNet (F-ConvNet) algorithm. We assessed the performance of our approach on the KITTI 3D object detection benchmark datasest under a wide variety of real-life scenarios. Experimental results suggest that F-ConvNet with our heuristic matches or improves upon the accuracy of original F-ConvNet while being significantly faster than F-ConvNet -- making it a viable approach to increase the accessibility of highly accurate real-time object detection to a variety of applications.

% % \addb{Bayzid: I made an attempt to rephrase the abstract (see above). But as I am not an expert in this domain, I am struggling to effectively capture the contribution of this work considering the state-of-the-art in 3d object detection. I would like to request you to finalize the abstract with Zahid during tomorrow's meeting.}



% % This paper proposes a \addr{our core contribution is not frustum based method. Instead focus on the mathematically challenging problem - approximate the frustum of interest that requires going from 2D to 3D with an increase of DOF by 1 that yields infinite number of solutions - for example, given a pixel in 2D we have an infinite number of possible solutions (mapped points in 3D), each with at a sample depth. Describe this with formal eigenvalue mathematics. There are infinite number of depth possible with infinitely small resolution. The core contribution to this work is to improve the performance by bounding the search within the most probable region of interest.} fast Frustum based method for 3D object detection using 2D images and 3D point clouds. Using state of the art object detectors we get object region proposals in 2D, which are used to generate frustums in the 3D point cloud for further processing using a 3D deep learning network \addb{this sentence describes a contribution which does not belong to us. Also, if this approach is especially for FconVnet, we may need to skip it. If it is a general approach for pointnet based methods, we may keep it after appropriate changes: Typically, frustums are generated from 2D region proposals, which are subsequently used for further processing ..}. \addb{Frustum generation is computationally challenging and have downstream impact on 3D object detection. Different sets of frustums may result in differential and perhaps in some cases less desirable outcomes both in terms of accuracy and running time. Therefore, the application of frustum-based approaches to real-time object detection is riddled with their computational challenges in generating a suitable set of frustums within a reasonable amount of time.} \addb{In this study, we have proposed an efficient heuristic to prune the 3D search space to effectively identify a set of ``frustums-of-interest''.} We are able to further narrow down our 3D search space using a heuristic based approach to find frustum of interest, which helps improve the run time of our model. \addb{Though simple, our proposed heuristic is highly efficient and effective. We have demonstrated the efficacy of our proposed approach by integrating this to the Frustrum ConvNet (F-ConvNet) algorithm, and we call the resulting architecture F-ConvNet Lite. We trained F-ConvNet Lite on the KITTI 3D object detection benchmark datasest and report the performance of F-ConvNet Lite on a variety of real-life scenarios. Experimental results suggest that F-ConvNet Lite is orders of magnitude faster than F-ConvNet (can we say precisely like 3-4 times faster?), making it a viable tool to increase the accessibility of real-time object detection to a variety of devices.} \addr{add more context on why we choose frustrum based model? Because ADAS (Automated Driver Assistance System) in most of the AV companies are already heavily relying on camera based detections but due to camera's inability to perceive the depth correctly the industry is increasingly relying on LiDAR as a an auxiliary sensor. For example, time to collision (TTC) detection is increasing using a camera and LiDAR fusion based models.} 

% % \addr{Question about ADAS and why we choose Frustrum model: Is it a good idea to be extreemely domain specific about the autonomous vehicle space? If So, is this something we should address in the abstract or intro?}

% % Based on the F-ConvNet algorithm, our model was designed to be smaller, faster and more efficient model increasing the accessibility of real-time object detection to a variety of devices. We train our model on the KITTI 3D object detection benchmarks and present our findings.
% % \addb{we need to mention the novelty more clearly and how it advances the state-of-the-art. We may want to say that our approach is generic and can be applied to other architectures, but we have demonstrated the efficacy of our proposed approache particularly on the F-ConvNet; Bayzid: I will be able to edit it more once I get a better picture of the overall contribution and experimental results.} \addr{specify the improvements with the precise numbers: what performance metrics were improved and and how much? Also, try to generalize this with any grid search systems including Voxel based methods. They also essentially do search on entire search space.}


OLD TABLES



% \begin{table}[!h]
% \caption{Car Only}
% \label{table-1}
% \begin{center}
% \begin{tabular}{|P{0.85cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|}
% \hline
% \multirow{2}{*}{\centering \textbf{Window}} & \multicolumn{3}{c|}{\textbf{BEV AP}}              & \multicolumn{3}{c|}{\textbf{3D AP}}               \\ \cline{2-7} 
%                                           & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} \\ \hline
% 2 & 87.952 & 87.246 & 86.459 & 82.611 & 74.921 & 73.832 \\ \hline
% 3 & 97.230 & 88.945 & 88.679 & 87.693 & 85.289 & 77.990 \\ \hline
% 4 & 96.800 & 88.790 & 88.691 & 86.731 & 85.009 & 77.770 \\ \hline
% 5 & 97.336 & 88.913 & 88.818 & 87.045 & 85.279 & 78.101 \\ \hline
% 7 & 97.542 & 89.455 & 89.218 & 87.268 & 86.051 & 78.457 \\ \hline
% 10 & 97.193 & 89.305 & 88.930 & 87.920 & 85.513 & 78.314 \\ \hline
% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[!h]
% \caption{Pedestrian AP in Pedestrian and Cyclist}
% \label{table-2}
% \begin{center}
% \begin{tabular}{|P{0.85cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|}
% \hline
% \multirow{2}{*}{\centering \textbf{Window}} & \multicolumn{3}{c|}{\textbf{BEV AP}}              & \multicolumn{3}{c|}{\textbf{3D AP}}               \\ \cline{2-7} 
%                                           & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} \\ \hline
% 2 & 51.848 & 55.922 & 50.316 & 47.979 & 47.023 & 47.684 \\ \hline
% 3 & 69.369 & 70.163 & 63.446 & 64.769 & 59.602 & 59.750 \\ \hline
% 4 & 72.777 & 72.505 & 65.556 & 69.125 & 62.658 & 62.242 \\ \hline
% 5 & 71.062 & 71.723 & 64.981 & 67.265 & 61.806 & 62.135 \\ \hline
% 7 & 72.580 & 72.343 & 65.148 & 68.908 & 62.894 & 62.514 \\ \hline
% 10 & 72.742 & 65.312 & 64.952 & 69.309 & 62.386 & 55.444 \\ \hline
% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[!h]
% \caption{Cyclist AP in Pedestrian and Cyclist}
% \label{table-3}
% \begin{center}
% \begin{tabular}{|P{0.85cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|}
% \hline
% \multirow{2}{*}{\centering \textbf{Window}} & \multicolumn{3}{c|}{\textbf{BEV AP}}              & \multicolumn{3}{c|}{\textbf{3D AP}}               \\ \cline{2-7} 
%                                           & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} \\ \hline
% 2 & 88.394 & 86.301 & 78.588 & 87.698 & 78.290 & 78.039 \\ \hline
% 3 & 90.350 & 89.211 & 88.645 & 89.375 & 87.642 & 79.359 \\ \hline
% 4 & 90.596 & 89.926 & 89.497 & 90.296 & 88.989 & 80.493 \\ \hline
% 5 & 89.526 & 88.834 & 88.151 & 85.971 & 85.889 & 77.640 \\ \hline
% 7 & 98.620 & 90.036 & 89.674 & 98.187 & 89.390 & 88.735 \\ \hline
% 10 & 89.965 & 88.803 & 88.280 & 89.717 & 87.969 & 79.731 \\ \hline
% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[!h]
% \caption{Car in Car-Pedestrian-Cyclist}
% \label{table-4}
% \begin{center}
% \begin{tabular}{|P{0.85cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|}
% \hline
% \multirow{2}{*}{\centering \textbf{Window}} & \multicolumn{3}{c|}{\textbf{BEV AP}}              & \multicolumn{3}{c|}{\textbf{3D AP}}               \\ \cline{2-7} 
%                                           & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} \\ \hline
% 2 & 88.856 & 87.655 & 86.909 & 84.681 & 75.877 & 74.791 \\ \hline
% 3 & 96.739 & 88.435 & 88.248 & 85.490 & 83.570 & 76.572 \\ \hline
% 4 & 97.225 & 89.003 & 88.913 & 86.308 & 84.840 & 77.868 \\ \hline
% 5 & 97.599 & 89.380 & 89.173 & 88.440 & 86.063 & 78.718 \\ \hline
% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[!h]
% \caption{Pedestrian in Car-Pedestrian-Cyclist}
% \label{table-5}
% \begin{center}
% \begin{tabular}{|P{0.85cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|}
% \hline
% \multirow{2}{*}{\centering \textbf{Window}} & \multicolumn{3}{c|}{\textbf{BEV AP}}              & \multicolumn{3}{c|}{\textbf{3D AP}}               \\ \cline{2-7} 
%                                           & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} \\ \hline
% 2 & 58.988 & 56.418 & 50.978 & 49.319 & 47.685 & 48.017 \\ \hline
% 3 & 67.936 & 62.274 & 62.669 & 64.119 & 59.295 & 53.187 \\ \hline
% 4 & 72.151 & 71.920 & 65.078 & 68.066 & 61.750 & 61.924 \\ \hline
% 5 & 68.687 & 69.508 & 63.128 & 64.370 & 59.545 & 59.911 \\ \hline
% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[!h]
% \caption{Cyclist in Car-Pedestrian-Cyclist}
% \label{table-6}
% \begin{center}
% \begin{tabular}{|P{0.85cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|}
% \hline
% \multirow{2}{*}{\centering \textbf{Window}} & \multicolumn{3}{c|}{\textbf{BEV AP}}              & \multicolumn{3}{c|}{\textbf{3D AP}}               \\ \cline{2-7} 
%                                           & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} \\ \hline
% 2 & 83.814 & 82.946 & 75.293 & 81.840 & 73.502 & 72.928 \\ \hline
% 3 & 89.509 & 88.611 & 88.004 & 88.933 & 87.543 & 86.989 \\ \hline
% 4 & 90.108 & 88.835 & 88.336 & 88.648 & 87.188 & 79.136 \\ \hline
% 5 & 89.386 & 88.361 & 87.986 & 88.178 & 86.244 & 78.301 \\ \hline
% \end{tabular}
% \end{center}
% \end{table}



% \begin{table}[!h]
% \caption{Car Only}
% \label{table-1}
% \begin{center}
% \begin{tabular}{|P{0.85cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|P{0.67cm}|P{1.02cm}|P{0.67cm}|}
% \hline
% \multirow{2}{*}{\centering \textbf{Window}} & \multicolumn{3}{c|}{\textbf{BEV AP}}              & \multicolumn{3}{c|}{\textbf{3D AP}}
% \\ \cline{2-7} 

% & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} \\ \hline

% 5 & 93.384 & 85.168 & 76.684 & 84.851 & 75.605 & 67.189 \\ \hline
% 7 & 89.697 & 88.109 & 79.457 & 86.771 & 77.724 & 76.033 \\ \hline
% 10 & 90.463 & 89.444 & 88.319 & 88.648 & 79.165 & 78.070 \\ \hline
% 15 & 98.005 & 89.411 & 88.640 & 88.640 & 86.245 & 78.626 \\ \hline
% 20 & 97.914 & 89.518 & 89.034 & 88.313 & 85.799 & 78.374 \\ \hline
% 25 & 97.643 & 88.947 & 88.582 & 87.405 & 85.135 & 77.863 \\ \hline
% 30 & 97.864 & 89.685 & 89.147 & 88.148 & 85.674 & 78.310 \\ \hline

% \end{tabular}
% \end{center}
% \end{table}




% \subsubsection{Gaussian Distribution}\label{sssec:5.1.2}
% In this approach we introduce a Gaussian distribution of floating point numbers, with mean set to 0 and standard deviation of 3, as error to the ground truth centers before feeding them into the model \addb{didn't understand this sentence...check the structure please}. Identical to \ref{sssec:5.1.1}, we test the performance of the model in KITTI evaluation protocol by setting windows of 2, 3, 5 and 10 meters around the augmented centers. The results once again establish that setting a window of 5 meters is the optimal choice 
%(TODO: Run tests and  add table).

% \subsubsection{Pseudo-random Integers}\label{sssec:5.1.1}
% In this approach we introduce pseudo-random integers in the interval [0, 3) as error to the ground truth centers before feeding them into the model. We test the performance of the model by setting window sizes 5, 7 and 10 meters around the augmented centers. We show the results of these experiments in Table-\ref{table-1} to Table-\ref{table-6} and observe that setting a window of 5 meter on either side of the augmented centers yields the least time-complexity without any significant reduction in accuracy.
% \subsubsection{Single Bucket Impact}\label{sssec:5.2.1}
% In this approach, for each point in the point cloud, we determine which bucket the point belongs to based on its depth. The point contributes a constant weight (the value is irrelevant) to that bucket. After the single pass through the point cloud, we sort the bins according to their weights and the bucket containing the highest weight is assumed to contain the center for our object of interest. We consider the arithmetic mean of the bucket-borders to be the center. This center is fed to the model and a window of 8 meters on either side of the estimated center is set to be iterated along the frustum axis. The results show a reasonable retention of accuracy while significantly reducing the search space 
% %(TODO: Run tests and add table).


% F-ConvNet \cite{wang_frustum_2019}  is an amodal 3D object detection architecture which, given 2D region proposals in an RGB image and a corresponding raw point cloud, generates a sequence of frustums from the point clouds and groups local points within those frustums. It aggregates the local point-wise features for use in a Fully Convolutional Network (FCN) to support end-to-end estimation of 3D bounding boxes. F-ConvNet uses a novel grouping mechanism - sliding frustums - to evaluate the frustum-enclosed portion of a raw point cloud iterating along the frustum axis. The frustum-level features are initially aggregated as 2D feature maps and later fed into a FCN, where they are down-sampled and up-sampled to generate a feature map that is fully-fused across the frustum axis. The downsides to sliding across the frustum axis is that a higher granularity of sliding directly leads to a proportionately worse run time. For the specific use cases and real-time applications like autonomous driving and vehicle tracking, this leads to a major impediment - a high computation cost owing to unnecessary iteration of the entire frustum axis that leads to poor real-time performances.
%This para is likely too long for the intro. We can use this info later though. 

% Fundamental to our approach is to efficiently estimate the depth of the object of interest within a frustum, which subsequently is used to constrain the frustum along the frustum axis and thereby reducing the 3D search space. Our approach to depth estimation uses point cloud density as an indicator of the possibility of the presence of an object. Combined with object bounding box information retrieved from RGB detectors, our heuristic provides acceptable accuracy while also having the advantage of being computationally inexpensive and generalizable to various use cases. Our approach is motivated by the autonomous driving use case but the heuristics and models can be extended to other related domains where latency sensitive accurate 3D object detection is necessary. 

%\addb{Our heuristic is a generic approach which can be used to make ... scalable.} 


%  \textbf{Generating Frustums from 2D region proposals} One of the major underlying assumptions of the F-ConvNet model is the availability of calibrated 2D images. These 2D images are used to generate 2D region proposals using state state of the art object detectors \cite{conf/eccv/LiuAESRFB16SSD, NIPS2015fasterrcnn}. Adjusting the camera coordinate system with the point cloud, the authors generate a series of  overlapping frustums by sliding a pair of parallel planes along the frustum axis with equal stride. Similarly, these frustums are generated for each 2D object proposal containing the object of interest, foreground and background points. 
%  \textbf{Feature extraction from Frustums through PointNet} For each region proposal from a RGB image, a sequence of $T$ frustums are generated by sliding along the frustum axis with a stride $s$. If there are $M$ points in each of these frustums, a three layer fully connected PointNet \cite{qi2016pointnet} is used to learn point wise features from each of these frustums. So, a total of $T$ PointNets with identical weights each output a 1D feature vector from each of the $T$ frustums for a single image. 
 
 
 
 
% In this work we propose 3D-FFS, a novel approach to make sensor fusion based 3D object detection networks significantly faster using a new class of heuristics. Existing sensor fusion models generate 3D region proposals by leveraging inferences from 2D object detectors. However, as images have no depth information, existing sensor fusion based models rely on extracting semantic features of points from the entire scene to locate the object. By leveraging aggregated intrinsic properties (e.g. point density) of the 3D point cloud data, 3D-FFS can substantially constrain the 3D search space and thereby significantly reduce training and inference time without sacrificing the accuracy. To demonstrate the efficacy of 3D-FFS, we have integrated it with Frustum ConvNet (F-ConvNet), one of the prominent sensor fusion based 3D object detection models.  We assessed the performance of 3D-FFS on the KITTI 3D object detection benchmark datasest. Experimental results suggest that 3D-FFS significantly reduces the inference and training time while making 2.03\% and 3.34\% improvements in accuracy for pedestrian and cyclist class, respectively. Moreover, our proposed approach improves the inference and training times of F-ConvNet by up to 56.80\% and 62.95\%, respectively, while reducing the memory usage by up to 58.53\%. 3D-FFS shows a lot of promise in domains with limited computing power, such as autonomous vehicles, drones, and robotics where LiDAR-Camera based sensor fusion perception systems are widely used.





% \section{Problem Definition}

% % Goal - 
% %     Classification & localization objects in 3D
% %     Faster Computation
% %     Define input & output
    
% % Input:2D image from Camera, 3D LiDAR point cloud

% % Output: representation of each object by a predefined class (say, k), amodal 3d bounding box (mention how we are representing the bounding box i.e. its parameters)

% % Add formulas and other representation details. 


% Our goal is classification and localization of objects in a 3D space given an input of RGB-D data. Our secondary goal is to ensure accurate 3D localization while ensuring real time performance. RGB image data is available in the form of images taken with a high resolution camera. The depth data is obtained from LiDAR sensors and is represented using a point cloud. The exact placement and specifications of the camera and LiDAR sensor is known. Based on this information, the point cloud is represented in RGB camera coordinates and a projection matrix is also known so that we can find the 3D frustum just from a 2D image region. Each object is represented by a class and an amodal 3D bounding box. The amodal box bounds the complete object even if part of the object is occluded or truncated.

% For each detected object, we must output the following: 
% \begin{itemize}
%     \item \textbf{Object Category: } The category of the object, represented by a class number (one among \textit{k} predefined classes). 
%     \item \textbf{3D Bounding Box:} The amodal 3D bounding box of the object, containing
%     \begin{enumerate}
%         \item  $\{x_c^g, y_c^g, z_c^g\}$ which denotes bounding box depth in the 3D coordinate system.
%         \item $\{l^g, w^g, h^g\}$ which denote length of the three sides. 
%         \item $\{\theta^g\}$ denotes yaw angle, which is the rotation perpendicular to the gravity direction. 
%     \end{enumerate}
% \end{itemize}

%-------------------------------------------------------------------------


 
% \begin{algorithm}[!h] 
% \caption{Identification Of High Density Bin} %TODO 
% \begin{algorithmic}[1] 
% \Function {Heuristic}{$frustum\_points$, $bin\_length$, $neighbor\_bins$} %TODO

%     \State $FD \leftarrow HashMap()$
    
%     \ForAll {$p \in frustum\_points$}
%         \State $bins \leftarrow \lfloor\frac{p.depth}{bin\_length}\rceil$
%         \State $FD(bin) \leftarrow FD(bin) + 1$
%         \For{$i\gets 1,  neighbor\_bins + 1$}
%             \State $FD(bin - i) \leftarrow FD(bin - i) + w$
%             \State $FD(bin + i) \leftarrow FD(bin + i) + w$
%         \EndFor
%     \EndFor
    
%     \State $depth \leftarrow max(FD) * bin\_length$
    
%     \State \textbf{return} $depth$
    
% \EndFunction
% \end{algorithmic} \label{Fig-Bin-Detection-Algo}
% \end{algorithm}

